A Local-Pattern Related Look-Up Table

This paper describes a Relevance-Zone pattern table (RZT) that can be used to replace a traditional transposition table. An RZT stores exact game values for patterns that are discovered during a Relevance-Zone-Based Search (RZS), which is the current state-of-the-art in solving L&D problems in Go. Positions that share the same pattern can reuse the same exact game value in the RZT. The pattern matching scheme for RZTs is implemented using a radix tree, taking into consideration patterns with different shapes. To improve the efficiency of table lookups, we designed a heuristic that prevents redundant lookups. The heuristic can safely skip previously queried patterns for a given position, reducing the overhead to 10% of the original cost. We also analyze the time complexity of the RZT both theoretically and empirically. Experiments show the overhead of traversing the radix tree in practice during lookup remain flat logarithmically in relation to the number of entries stored in the table. Experiments also show that the use of an RZT instead of a traditional transposition table significantly reduces the number of searched nodes on two data sets of 7x7 and 19x19 L&D Go problems.

==> backup/MCTS_and_FTL.tex <==
{\color{red}
AlphaZero \citep{silver2018general} is a general reinforcement learning algorithm that can achieve super-human level playing strength for games without requiring any expert domain knowledge.

The training routine consists of two phases: self-play and optimization.
In a nutshell, a two-headed neural network that outputs a policy distribution $p$ and a value scalar $v$ is periodically optimized with data that is collected via self-play.
Self-play games are generated by running a set number of MCTS simulations with the most recently optimized neural network.
In order to explore the game state space more thoroughly during self-play, Dirichlet noise Dir($\alpha$) is added to $p$ specifically for the MCTS root node.
In the optimization phase, random positions are sampled from the latest self-play games, where the network is optimized by the following loss function:
\begin{equation}
\label{equ:Alphazero_loss}
    L=(z-v)^2 - \pi^{\rm{T}} \log p + c\Vert\theta\Vert^2,
\end{equation}
where $z$ is the ground truth outcome of the game for that position, $\pi$ is the MCTS search distribution, $c$ is an L2 regularization weight, and $\theta$ represents the network parameters.
As mentioned above, the optimized network will then be used to generate the next round of self-play games.

An AlphaZero-like training method called {\em Faster to Life (FTL)} \citep{shih2022anovel}, by modifying the goal of the AlphaZero algorithm so that it prefers winning in fewer moves.
With FTL, we defined the winning condition to be White achieving UCA for any number of stones within $d$ moves from the current position. 
For example, with $d=20$, White wins only if it is able to reach UCA within 20 moves.
Given multiple values of $d$, the problem setting is similar to determining win/loss with multiple komi values, which can be handled with multi-labelled value networks \citep{wu2018multilabeled}.

Given a position $p$, the value network head outputs a set of additional $d$-win rates (the rates of winning within $d$ moves), where $d$ ranges from $1$ to a sufficiently large number. 
Namely, for all positions $p$ during the self-play portion of AlphaZero training, if White lives by UCA at the $d$-th move from the current position, we count one more $d'$-win for all $d' \geq d$, but not for all $d'<d$. 
These $d'$-wins are used to update the set of $d$-win rates of $p$. 
Hence, White tends to win faster if their $d$-win rates are high for low values of $d$.
}
The FTL has shown that it has better performance than vanilla AlphaZero when solving L\&D problems.\citep{shih2022anovel},

==> backup/abtract_old.tex <==
Pattern matching is common issues that most board games researcher has faced.
The Relevance-Zone Based Seach (RZS) can search for patterns to conclude that a player is a win.
The traditional way to treat them as wins and lookup by hashing as transposition tables does not work for its different shapes and size.
Therefore, we proposed a data structure that is based on radix trees to improve the performance about 80\% for the look-up times.
The experiments has shown that RZ matching scheme has improved simulation counts for four times on two data sets of $7 \times 7$ and $19 \times 19$ L\&D problem of Go.
Finally, we discuss some opening issues about matching zone patterns.

==> backup/author_old.tex <==
\ifieee
\author{

\IEEEauthorblockN{
Chung-Chin Shih$^{a,d}$, 
Ting Han Wei$^{b}$, 
Ti-Rong Wu$^{c}$, and
I-Chen Wu$^{a}$
} \\
\IEEEauthorblockA{$^{a}$Department of Computer Science, National Yang Ming Chiao Tung University, Hsinchu, Taiwan
\\rockmanray@aigames.nctu.edu.tw, icwu@cs.nctu.edu.tw} \\
\IEEEauthorblockA{$^{b}$Department of Computing Science, University of Alberta, Edmonton, Canada
\\tinghan@ualberta.ca} \\    
\IEEEauthorblockA{$^{c}$Institute of Information Science, Academia Sinica, Taipei, Taiwan 
\\tirongwu@iis.sinica.edu.tw} \\
\IEEEauthorblockA{$^{d}$Research Center for IT Innovation, Academia Sinica, Taipei, Taiwan 
\\icwu@citi.sinica.edu.tw} 

\thanks{
Manuscript received X X, 2022.
This research is partially supported by the National Science and Technology Council (NSTC) of the Republic of China (Taiwan) under Grant Number 110-2221-E-A49-067-MY3 and 110-2634-F-A49-004; the Higher Education Sprout Project of the National Yang Ming Chiao Tung University and Ministry of Education (MOE), Taiwan. The computing resource is partially supported by National Center for High-performance Computing (NCHC), Taiwan. (Corresponding author: I-Chen Wu.)
}
}
\fi

==> backup/rockmanray.tex <==
% rockmanray: the following has no significant improvements
\begin{comment}
\subsubsection{Skip Larger Zone Patterns}
\label{subsubsec:skip_larger_zone_patterns}
In the previous statements, we note that the position $p$ and RZ attern $\phi$ are many-to-many mapping.
In the usage of RZ, smaller RZs can incur more pruning, therefore we disable a zone pattern $e_1$ is a zone pattern $e_2$ is just a subset of $e_1$.
\end{comment}
